Continuous Evolution of Digital Twins using the DarTwin Notation

Despite best efforts, various challenges remain in the creation and maintenance processes of digital twins (DTs). One of those primary challenges is the constant, continuous and omnipresent evolution of systems, their user's needs and their environment, demanding the adaptation of the developed DT systems. DTs are developed for a specific purpose, which generally entails the monitoring, analysis, simulation or optimization of a specific aspect of an actual system, referred to as the actual twin (AT). As such, when the twin system changes, that is either the AT itself changes, or the scope/purpose of a DT is modified, the DTs usually evolve in close synchronicity with the AT. As DTs are software systems, the best practices or methodologies for software evolution can be leveraged. This paper tackles the challenge of maintaining a (set of) DT(s) throughout the evolution of the user's requirements and priorities and tries to understand how this evolution takes place. In doing so, we provide two contributions: (i) we develop DarTwin, a visual notation form that enables reasoning on a twin system, its purposes, properties and implementation, and (ii) we introduce a set of architectural transformations that describe the evolution of DT systems. The development of these transformations is driven and illustrated by the evolution and transformations of a family home's DT, whose purpose is expanded, changed and re-prioritized throughout its ongoing lifecycle. Additionally, we evaluate the transformations on a lab-scale gantry crane's DT.

==> figures/plots/arbiter.tex <==
% Arrow styles: specialization contributes relation flow

\begin{scope}[xshift=-4cm,yshift=-2em]
    \input{figures/plots/parts/energy-saving-inner}
\end{scope}

\draw[relation] (heater) .. controls ([yshift=6cm,xshift=3cm]heater) and ([yshift=.5cm,xshift=3cm]energy poi) .. (energy poi);

\begin{scope}[on behind layer]
    \node[langDT,fit=(lowerenergy goal) (presence poi)(whenpresent goal)(whenabsent goal)(energy poi),label={[below]north:Energy Saving DT}] (dt2) {};
\end{scope}

% freeze protect
\node[goal,right=3.5 of comfort goal,yshift=-2em] (freezeprotect goal) {Freeze\\protection};
\draw[contributes] (temperature poi) -- (freezeprotect goal);

\begin{scope}[on behind layer]
    \node[langDT,,yshift=.5em,fit=(temperature poi) (freezeprotect goal),label={[below]north:{Freeze Protect DT}}] {};
\end{scope}

\node[process,above right=2 and -.5 of heater] (dt3 process) {Freeze Protect DT};
\draw[flow] (dt3 process) -- (heater);
% \draw[flow] (temperature sensor.110) |- (dt3 process.north west);
\draw[flow] (temperature sensor.east) -- ++(2.5cm,0) -- (dt3 process.south west);


% cost stuff
\node[goal,highlightnode, left=2 of whenabsent goal] (cost goal) {Save\\Money};
\node[mvar,highlightnode,below=1 of cost goal] (cost poi) {Hourly Energy\\Prices};
\draw[contributes,highlight] (cost poi) -- (cost goal);

\begin{scope}[on background layer]
    \node[langDT,highlight, fit=(cost poi)(cost goal),label={[below]north:{Cost Saving DT}}] (dt2) {};
\end{scope}

% \node[goal,highlightnode, below right=0.35 and .9 of dt2.south] (arbiter goal) { Reduce Energy+Comfort\\Harmonization (Arbiter)};
% \draw[specialization,highlight] (arbiter goal.60) -- ++(0,2cm) -- (cost goal);
% \draw[specialization,highlight] (arbiter goal.60) |- (lowerenergy goal.west);

\draw[conflict,highlight] (cost goal) -- (lowerenergy goal);

% DT 2 + presence sensor

\node[process,left=3 of dt1 process] (dt2 process) {Energy Saving DT};
\node[sensor] (presence sensor) at (dt2 process |- temperature sensor) {Presence\\Sensor};
\node[process,highlightnode,above=1 of dt2 process] (cost process) {Cost Saving DT};

\node[process,highlightnode,above right=0 and .75 of dt2 process] (arbiter process) {Arbiter};

% arrows
\draw[flow,highlight] (dt2 process) |-  (arbiter process.190);
\draw[flow,highlight] (cost process) |-  (arbiter process.170);
\draw[flow,highlight] (arbiter process) -|  (dt1 process);

\draw[flow] (presence sensor) -- (dt2 process);
\draw[flow] (room AT.north -| presence sensor) -- (presence sensor);


\node[sensor, highlightnode, left=1.5 of cost process] (cost sensor) {Cost Price\\Table};
\draw[flow,highlight] (cost sensor) -- (cost process);
\draw[relation,highlight] (cost sensor) to[out=120,in=270] (cost poi);


\draw[relation] (presence sensor.west) .. controls ([xshift=-3cm] dt2 process.west) and ([yshift=2cm] dt2 process.east) .. (presence poi.south);

% refactored  DT1
\begin{scope}[on behind layer]
    \node[sys,fill=gray!10,fit=(dt1 process) (dt2 process) (cost process)(cost process),label={[below]north:{Energy \& Cost Saving Warm Comfort DT}}] (dt1-system) {};
\end{scope}

\begin{scope}[on background layer]
    \node[sys, fit=(temperature sensor)(cost sensor)(room AT)(dt1-system)(heater)(dt3 process),label={[below]north:{Energy \& Cost Saving Safe Warm Comfort Twin System}}] {};
\end{scope}

\draw[flow] (dt1-system) -- (dt3 process);




==> figures/plots/co2-complete.tex <==
% Arrow styles: specialization contributes relation flow

\begin{scope}[xshift=-4cm,yshift=-2em]
    \input{figures/plots/parts/energy-saving-inner}
\end{scope}

\draw[relation] (heater) .. controls ([yshift=6cm,xshift=3cm]heater) and ([yshift=.5cm,xshift=3cm]energy poi) .. (energy poi);

\begin{scope}[on behind layer]
    \node[langDT,fit=(lowerenergy goal) (presence poi)(whenpresent goal)(whenabsent goal)(energy poi),label={[below]north:Energy Saving DT}] (dt2) {};
\end{scope}

% freeze protect
\node[goal,right=3.5 of comfort goal,yshift=-2em] (freezeprotect goal) {Freeze\\protection};
\draw[contributes] (temperature poi) -- (freezeprotect goal);

\begin{scope}[on behind layer]
    \node[langDT,yshift=.5em,fit=(temperature poi) (freezeprotect goal),label={[below]north:{Freeze Protect DT}}] {};
\end{scope}

\node[process,above right=2 and -.5 of heater] (dt3 process) {Freeze Protect DT};
\draw[flow] (dt3 process) -- (heater);
% \draw[flow] (temperature sensor.110) |- (dt3 process.north west);
\draw[flow] (temperature sensor.east) -- ++(2.5cm,0) -- (dt3 process.south west);


% cost stuff
\node[goal, left=2 of whenabsent goal] (cost goal) {Save\\Money};
\node[mvar,below=1.5 of cost goal] (cost poi) {Hourly Energy\\Prices};
\draw[contributes] (cost poi) -- (cost goal);

\begin{scope}[on background layer]
    \node[langDT, fit=(cost poi)(cost goal),label={[below]north:{Cost Saving DT}}] (dt2) {};
\end{scope}

% \node[goal, below right=0.35 and .9 of dt2.south] (arbiter goal) {Arbiter};
% \draw[specialization] (arbiter goal.60) -- ++(0,2cm) -- (cost goal);
% \draw[specialization] (arbiter goal.60) |- (lowerenergy goal.west);
\draw[conflict] (cost goal) -- (lowerenergy goal);
% DT 2 + presence sensor

\node[process,left=3 of dt1 process] (dt2 process) {Energy Saving DT};
\node[sensor,below=1.25 of dt2 process] (presence sensor) {Presence\\Sensor};
\node[process,above=1 of dt2 process] (cost process) {Cost Saving DT};

\node[process,above right=0 and .75 of dt2 process] (arbiter process) {Arbiter};

% arrows
\draw[flow] (dt2 process) |-  (arbiter process.190);
\draw[flow] (cost process) |-  (arbiter process.170);
\draw[flow] (arbiter process) -|  (dt1 process);

\draw[flow] (presence sensor) -- (dt2 process);
\draw[flow] (room AT) -| (presence sensor);


\node[sensor, left=1.5 of cost process] (cost sensor) {Cost Price\\Table};
\draw[flow] (cost sensor) -- (cost process);
\draw[relation] (cost sensor) to[out=120,in=270] (cost poi);


\draw[relation] (presence sensor.west) .. controls ([xshift=-3cm] dt2 process.west) and ([yshift=2cm] dt2 process.east) .. (presence poi.south);

% refactored  DT1
\begin{scope}[on behind layer]
    \node[sys,fill=gray!10,fit=(dt1 process) (dt2 process) (cost process)(cost process),label={[below]north:{Energy \& Cost Saving Warm Comfort DT}}] (dt1-system) {};
\end{scope}

\draw[flow] (dt1-system) -- (dt3 process);



% CO2 stuff
\node[goal, left=3.5 of cost goal] (co2 goal) {Fresh Air};
\node[mvar,below left=.75 and .45 of co2 goal.south] (co2 poi) {CO$_2$\\Level};
\node[mvar,below right=.75 and .45 of co2 goal.south] (outsidetemp poi) {Outside\\Temperature};
\draw[contributes] (co2 poi) -- (co2 goal);

% \draw[contributes] ( poi) -- (co2 goal);

\begin{scope}[on background layer]
    \node[langDT,fit=(co2 poi)(co2 goal)(outsidetemp poi),label={[below]north:{Fresh Air DT}}] (co2dt) {};
\end{scope}


\draw[conflict,highlight] (co2 goal) -- (lowerenergy goal) node[pos=.15,inner sep=0em] (mid) {};
\draw[contributes,highlight] (outsidetemp poi) -- (mid);


% \node[mvar,below=2.5 of co2 goal.south] (numpeople poi) {\# people};
% \draw[contributes] (numpeople poi) -- (co2 poi);
% \draw[contributes] (numpeople poi) .. controls ([xshift=-.7cm,yshift=1cm] cost poi) .. (presence poi);


\node[actuator, below right=0.5 and 1 of room AT] (ventilation) {Ventilation};
\node[sensor] (co2 sensor) at (ventilation -| temperature sensor){CO$_2$ Sensor};
\node[process, below=2 of room AT] (co2 process) {Fresh Air DT};

\draw[flow] (room AT) -| (co2 sensor);
\draw[flow] (co2 sensor) |- (co2 process);
\draw[flow] (co2 process) -| (ventilation);
\draw[flow] (ventilation) |- (room AT);

\node[sensor] (outsidetemp sensor) at (presence sensor -| cost sensor){Outside\\Temperature Sensor};
\draw[flow] (outsidetemp sensor) |- (co2 process);

\draw[flow] (co2 process.south) -- ++(0,-.25) -| ([xshift=-1cm]outsidetemp sensor.west) |- (arbiter process);



\draw[relation] (co2 sensor) .. controls ([xshift=-10cm]co2 sensor) and ([yshift=-10cm]co2 poi) .. (co2 poi);

\draw[relation] (outsidetemp sensor) to[in=270,out=130] (outsidetemp poi);



\begin{scope}[on background layer]
    \node[sys, fit=(temperature sensor)(cost sensor)(room AT)(dt1-system)(heater)(dt3 process)(outsidetemp sensor)(co2 process),label={[below]north:{Energy \& Cost Saving Fresh Air Safe Warm Comfort Twin System}}] {};
\end{scope}

==> figures/plots/co2.tex <==
% Arrow styles: specialization contributes relation flow

\begin{scope}[xshift=-4cm,yshift=-2em]
    \input{figures/plots/parts/energy-saving-inner}
\end{scope}

\draw[relation] (heater) .. controls ([yshift=6cm,xshift=3cm]heater) and ([yshift=.5cm,xshift=3cm]energy poi) .. (energy poi);

\begin{scope}[on behind layer]
    \node[langDT,fit=(lowerenergy goal) (presence poi)(whenpresent goal)(whenabsent goal)(energy poi),label={[below]north:Energy Saving DT}] (dt2) {};
\end{scope}

% freeze protect
\node[goal,right=3.5 of comfort goal,yshift=-2em] (freezeprotect goal) {Freeze\\protection};
\draw[contributes] (temperature poi) -- (freezeprotect goal);

\begin{scope}[on behind layer]
    \node[langDT,yshift=.5em,fit=(temperature poi) (freezeprotect goal),label={[below]north:{Freeze Protect DT}}] {};
\end{scope}

\node[process,above right=2 and -.5 of heater] (dt3 process) {Freeze Protect DT};
\draw[flow] (dt3 process) -- (heater);
% \draw[flow] (temperature sensor.110) |- (dt3 process.north west);
\draw[flow] (temperature sensor.east) -- ++(2.5cm,0) -- (dt3 process.south west);


% cost stuff
\node[goal, left=2 of whenabsent goal] (cost goal) {Save\\Money};
\node[mvar,below=1.5 of cost goal] (cost poi) {Hourly Energy\\Prices};
\draw[contributes] (cost poi) -- (cost goal);

\begin{scope}[on background layer]
    \node[langDT, fit=(cost poi)(cost goal),label={[below]north:{Cost Saving DT}}] (dt2) {};
\end{scope}

% \node[goal, below right=0.35 and .9 of dt2.south] (arbiter goal) {Arbiter};
% \draw[specialization] (arbiter goal.60) -- ++(0,2cm) -- (cost goal);
% \draw[specialization] (arbiter goal.60) |- (lowerenergy goal.west);

\draw[conflict] (cost goal) -- (lowerenergy goal);

% DT 2 + presence sensor

\node[process,left=3 of dt1 process] (dt2 process) {Energy Saving DT};
\node[sensor] (presence sensor) at (dt2 process |- temperature sensor) {Presence\\Sensor};
\node[process,above=1 of dt2 process] (cost process) {Cost Saving DT};

\node[process,above right=0 and .75 of dt2 process] (arbiter process) {Arbiter};

% arrows
\draw[flow] (dt2 process) |-  (arbiter process.190);
\draw[flow] (cost process) |-  (arbiter process.170);
\draw[flow] (arbiter process) -|  (dt1 process);

\draw[flow] (presence sensor) -- (dt2 process);
\draw[flow] (room AT.north -| presence sensor) -- (presence sensor);


\node[sensor, left=1.5 of cost process] (cost sensor) {Cost Price\\Table};
\draw[flow] (cost sensor) -- (cost process);
\draw[relation] (cost sensor) to[out=120,in=270] (cost poi);


\draw[relation] (presence sensor.west) .. controls ([xshift=-3cm] dt2 process.west) and ([yshift=2cm] dt2 process.east) .. (presence poi.south);

% refactored  DT1
\begin{scope}[on behind layer]
    \node[sys,fill=gray!10,fit=(dt1 process) (dt2 process) (cost process)(cost process),label={[below]north:{Energy \& Cost Saving Warm Comfort DT}}] (dt1-system) {};
\end{scope}

\draw[flow] (dt1-system) -- (dt3 process);



% CO2 stuff
\node[goal,highlightnode, left=2 of cost goal] (co2 goal) {Fresh Air};
\node[mvar,highlightnode,below=.75 of co2 goal.south] (co2 poi) {CO$_2$\\Level};
% \node[mvar,highlightnode,below right=.75 and .45 of co2 goal.south] (outsidetemp poi) {Outside\\Temperature};
\draw[contributes,highlight] (co2 poi) -- (co2 goal);

% \draw[contributes,highlight] ( poi) -- (co2 goal);

\begin{scope}[on background layer]
    \node[langDT,highlight,fit=(co2 poi)(co2 goal),label={[below]north:{Fresh Air DT}}] (co2dt) {};
\end{scope}

% \draw[conflict,highlight] (co2 goal) -- (lowerenergy goal) node[pos=.15,inner sep=0em] (mid) {};
% \draw[contributes,highlight] (outsidetemp poi) -- (mid);

% \node[mvar,highlightnode,below=2.5 of co2 goal.south] (numpeople poi) {\# people};
% \draw[contributes,highlight] (numpeople poi) -- (co2 poi);
% \draw[contributes,highlight] (numpeople poi) .. controls ([xshift=-.7cm,yshift=1cm] cost poi) .. (presence poi);


\node[process,highlightnode, left=5 of dt2 process] (co2 process) {Fresh Air DT};
\node[sensor,highlightnode, below left=0.5 and .5 of co2 process] (co2 sensor) {CO$_2$ Sensor};
\node[actuator,highlightnode, below right=0.5 and .5 of co2 process] (ventilation) {Ventilation};

\draw[flow,highlight] (room AT.north -| co2 sensor) -| (co2 sensor);
\draw[flow,highlight] (co2 sensor) |- (co2 process);
\draw[flow,highlight] (co2 process) -| (ventilation);
\draw[flow,highlight] (ventilation) -- (room AT.north -| ventilation);

% \node[sensor,highlightnode] (outsidetemp sensor) at (presence sensor -| cost sensor){Outside\\Temperature Sensor};
% \draw[flow,highlight] (outsidetemp sensor) |- (co2 process);

% \draw[flow,highlight] (co2 process.south) - (arbiter process);



\draw[relation,highlight] (co2 sensor.150) to[out=90,in=240] (co2 poi);
\draw[relation,highlight] (co2 poi) to[out=300,in=90] (ventilation.30);

% \draw[relation,highlight] (outsidetemp sensor) to[in=270,out=130] (outsidetemp poi);



\begin{scope}[on background layer]
    \node[sys, fit=(temperature sensor)(cost sensor)(room AT)(dt1-system)(heater)(dt3 process)(co2 process),label={[below]north:{Energy \& Cost Saving Fresh Air Safe Warm Comfort Twin System}}] {};
\end{scope}

==> figures/plots/freeze-protect-refactored.tex <==
% % Arrow styles: specialization contributes relation flow

% \begin{scope}
%     \input{figures/plots/parts/energy-saving-complete}
% \end{scope}

% % refactored  DT1
% \begin{scope}[on behind layer]
%     \node[sys,fill=gray!10,fit=(dt1 process) (dt2 process),label={[below]north:{Energy Saving Warm Comfort DT}},xshift=.5em] (dt1-system) {};
% \end{scope}


% % freeze protect
% \node[goal,right=3.5 of comfort goal,yshift=-2em] (freezeprotect goal) {Freeze\\protection};
% \draw[contributes] (temperature poi) -- (freezeprotect goal);

% \begin{scope}[on behind layer]
%     \node[langDT,yshift=0.5em,fit=(temperature poi) (freezeprotect goal),label={[below]north:{Freeze Protect DT}}] {};
% \end{scope}


% \node[process,highlightnode,above right=2 and -.5 of heater] (dt3 process) {Freeze Protect DT};

% \draw[flow,highlight] ([xshift=10pt,yshift=2pt]dt3 process.south west) -- (heater);
% \draw[flow,highlight] (dt1-system.east) -- ([xshift=2pt,yshift=2pt]dt3 process.south west);


% % \draw[flow] (temperature sensor.110) |- (dt3 process);
% \draw[flow] (temperature sensor.east) -- ++(2.5cm,0) -- (dt3 process.south west);

% \draw[relation] (presence sensor.west) .. controls ([xshift=-3cm] dt2 process.west) and ([yshift=2cm] dt2 process.east) .. (presence poi.south);



% \begin{scope}[on background layer]
%     \node[sys, fit=(temperature sensor)(room AT)(dt1-system)(heater)(dt3 process),label={[below]north:{Energy Saving Safe Warm Comfort Twin System}}] {};
% \end{scope}




==> figures/plots/freeze-protect.tex <==
% Arrow styles: specialization contributes relation flow

\begin{scope}
    \input{figures/plots/parts/energy-saving-complete}
\end{scope}

% refactored  DT1
\begin{scope}[on behind layer]
    \node[sys,fill=gray!10,fit=(dt1 process) (dt2 process),label={[below]north:{Energy Saving Warm Comfort DT}},xshift=.5em] (dt1-system) {};
\end{scope}


% freeze protect
\node[goal,highlightnode,right=3.54 of comfort goal,yshift=-2em] (freezeprotect goal) {Freeze\\protection};
\draw[contributes,highlight] (temperature poi) -- (freezeprotect goal);

\node[process,highlightnode,above right=2 and -.5 of heater] (dt3 process) {Freeze Protect DT};
\draw[flow,highlight] (dt3 process) -- (heater);

% \draw[flow,highlight] (temperature sensor.110) |- (dt3 process);
\draw[flow,highlight] (temperature sensor.east) -- ++(2.5cm,0) -- (dt3 process.south west);

\draw[relation] (presence sensor.west) .. controls ([xshift=-3cm] dt2 process.west) and ([yshift=2cm] dt2 process.east) .. (presence poi.south);



\begin{scope}[on background layer]
    \node[sys, fit=(temperature sensor)(room AT)(dt1-system)(heater)(dt3 process),label={[below]north:{Energy Saving Safe Warm Comfort Twin System}}] {};
\end{scope}


\begin{scope}[on behind layer]
    \node[langDT,yshift=.5em,highlight,fit=(temperature poi) (freezeprotect goal),label={[below]north:{Freeze Protect DT}}] {};
\end{scope}






==> figures/plots/lower-energy-cost-digital-twin.tex <==
% Arrow styles: specialization contributes relation flow

\begin{scope}[on behind layer]
    \node[sys, fit=(temperature sensor)(dt1 process) (room AT)(heater),fill=gray!10,label={[below]north:{Warm Comfort Twin System}}] (dt1-system) {};
\end{scope}

\begin{scope}[xshift=-4cm,yshift=-2em]
    \input{figures/plots/parts/energy-saving-inner}
\end{scope}

\draw[relation] (heater) .. controls ([yshift=6cm,xshift=3cm]heater) and ([yshift=.5cm,xshift=3cm]energy poi) .. (energy poi);


\begin{scope}[on behind layer]
    \node[langDT,highlight,fit=(lowerenergy goal) (presence poi)(whenpresent goal)(whenabsent goal)(energy poi),label={[below]north:Energy Saving DT}] (dt2) {};
\end{scope}



% DT 2 + presence sensor

\node[process,highlightnode,left=3 of dt1 process] (dt2 process) {Energy Save DT};
\node[sensor,highlightnode] (presence sensor) at (dt2 process |- temperature sensor) {Presence\\Sensor};

% arrows
\draw[flow,highlight] (dt2 process) |- ($(dt2 process.north)+(0,0.5)$) -| (dt1 process);
\draw[flow,highlight] (presence sensor) -- (dt2 process);
\draw[flow,highlight] (room AT) -| (presence sensor);

\draw[relation,highlight] (presence sensor.west) .. controls ([xshift=-3cm,yshift=1cm] dt2 process.west) and ([yshift=2cm,xshift=1cm] dt2 process.east) .. (presence poi.south);

\begin{scope}[on background layer]
    \node[sys, fit=(temperature sensor)(dt2 process)(dt1-system),label={[below]north:{Energy Saving Warm Comfort Twin System}}] {};
\end{scope}

==> figures/plots/lower-energy-cost-reasoning.tex <==
% Arrow styles: specialization contributes relation flow

% \begin{scope}[on behind layer]
%     \node[sys, fit=(dt1 process) (room AT),fill=gray!10,label={[below]north:{Warm Comfort Twin System}}] (dt1-system) {};
% \end{scope}



% \node[goal,highlightnode,below=1.25 of whenabsent goal] (lowerenergy goal) {Lower Energy\\Usage};

% \node[mvar,highlightnode,below left=0.5 and -.25 of whenpresent goal] (presence poi) {Presence of\\People};
% \node[evar,highlightnode,below=0.5 of lowerenergy goal] (energy poi) {Energy};

\draw[specialization,highlight] (whenabsent goal.north)  |- ($(whenabsent goal.north)+(0,1em)$) -| (lowerenergy goal);

\draw[specialization,highlight] (whenpresent goal.north) |- ($(whenpresent goal.north)+(0,1em)$) -| (lowerenergy goal);

% \draw[contributes,highlight] (presence poi) -- (whenpresent goal);
% \draw[contributes,highlight] (presence poi) -- (whenabsent goal);
% \draw[contributes,highlight] (whenabsent goal) -- (lowerenergy goal);

% \draw[contributes,highlight] (energy poi) -- (lowerenergy goal);

% \draw[relation,highlight] (heater) .. controls ([yshift=6cm,xshift=3cm]heater) and ([yshift=.5cm,xshift=3cm]energy poi) .. (energy poi);




==> figures/plots/parts/comfort-goal.tex <==
% above the line
\node[goal] (comfort goal) {\textbf{Comfort}\\t: Temp [l,u]};
% \node[cmvar,below=1 of comfort goal] (temperature poi) {Room\\Temperature};

% arrows
% \draw[contributes] (temperature poi) -- (comfort goal);

% \begin{scope}[on behind layer] % (temperature poi) 
%     \node[langDT,fit=(comfort goal),label={[below]north:Thermo Logic DT}] (dt1) {};
% \end{scope}



==> figures/plots/parts/energy-saving-complete.tex <==
% \begin{scope}[xshift=-4cm,yshift=-2em]
%     \input{figures/plots/parts/energy-saving-inner}
% \end{scope}

% \draw[relation] (heater) .. controls ([yshift=6cm,xshift=3cm]heater) and ([yshift=.5cm,xshift=3cm]energy poi) .. (energy poi);

% \begin{scope}[on behind layer]
%     \node[langDT,fit=(lowerenergy goal) (presence poi)(whenpresent goal)(whenabsent goal)(energy poi),label={[below]north:Energy Saving DT}] (dt2) {};
% \end{scope}



% % DT 2 + presence sensor

% \node[process,left=3 of dt1 process] (dt2 process) {Energy Saving DT};
% \node[sensor] (presence sensor) at (dt2 process |- temperature sensor) {Presence\\Sensor};

% % arrows
% \draw[flow] (dt2 process) |- ($(dt2 process.north)+(0,0.5)$) -| (dt1 process);
% \draw[flow] (presence sensor) -- (dt2 process);
% \draw[flow] (room AT.north -| presence sensor) -- (presence sensor);

% \draw[relation] (presence sensor.west) .. controls ([xshift=-3cm] dt2 process.west) and ([yshift=2cm] dt2 process.east) .. (presence poi.south);


==> figures/plots/parts/energy-saving-inner.tex <==

\node[goal] (whenpresent goal) {Comfort\\When Present};
\node[goal,left=1 of whenpresent goal] (whenabsent goal) {Comfort\\When Absent};
\node[goal,below=1.25 of whenabsent goal] (lowerenergy goal) {Lower Energy\\Usage};

\node[mvar,below left=0.5 and -.25 of whenpresent goal] (presence poi) {Presence of\\People};
\node[evar,below=0.5 of lowerenergy goal] (energy poi) {Energy};

\draw[specialization] (whenabsent goal.north)  |- (comfort goal);

\draw[specialization] (whenpresent goal.north) |- (comfort goal);

\draw[contributes] (presence poi) -- (whenpresent goal);
\draw[contributes] (presence poi) -- (whenabsent goal);
\draw[contributes] (whenabsent goal) -- (lowerenergy goal);

\draw[contributes] (energy poi) -- (lowerenergy goal);

==> figures/plots/parts/parts.tex <==
\newcommand{\comfortdt}[#1]{
% DT1 + ports
\node[process,#1,minimum width=3cm] (dt1 process) {Comfort DT};
\node[port,label={below:{\scriptsize }}] (dt1-heater-port) at (dt1 process.east) {$\rightarrow$};
\node[port,label={below:{\scriptsize }}] (dt1-comfort-temp-port) at (dt1 process.west) {$\rightarrow$};
\node[port,label={below:{\scriptsize }}] (dt1-temp-port) at (dt1 process.south) {$\uparrow$};
}

==> figures/plots/parts/rectangle.tex <==


% Room AT + ports
\node[actualtwin,minimum width=6cm,minimum height=1.75cm] (room AT) at (0,-2.5) {\large Room AT};
\node[port,label={below:{\scriptsize Room Temperature}}] (room-temp-port) at (room AT.north) {$\uparrow$};
\node[port,label={below:{\scriptsize Heater}}] (room-heater-port) at (room AT.22) {$\downarrow$};


% below the line
% \node[process] (dt1 process) {Thermo\\Logic DT};
% \node[port,label={below:{\tiny Heater}}] (dt1-heater-port) at (dt1 process.east) {$\rightarrow$};
% \node[port,label={below:{\tiny Heater}}] (dt1-temp-port) at (dt1 process.south) {$\uparrow$};


% \node[actuator, below right=0.5 and 1 of dt1 process] (heater) {Heater};
% \node[sensor,below left=0.5 and 1 of dt1 process] (temperature sensor) {Temperature\\Sensor};

% % arrows
% \draw[flow] (temperature sensor) |- (dt1 process);
% \draw[flow] (room AT.north -| temperature sensor.south) -- (temperature sensor);
% \draw[flow] (heater) -- (room AT.north -| heater.south);


% trivial thermo connections
% \draw[relation] (temperature sensor.110) to[out=110, in=200] (temperature poi);
% \draw[relation] (temperature poi) to[out=-30,in=45] (heater.east);


==> figures/plots/parts/separation.tex <==

% separation line
\node[label] (influences label) at (6,0) {Goals and \Acs{poi}};
\node[label,below=0.5 of influences label] (implementation) {Implementation};
\draw[separationLine] ($(influences label.south east)+(.5,-.25)$) -- ++(-13,0);



==> figures/plots/refactored-lower-energy-comfort.tex <==
% Arrow styles: specialization contributes relation flow

\begin{scope}
    \input{figures/plots/parts/energy-saving-complete}
\end{scope}

% refactored  DT1
\begin{scope}[on behind layer]
    \node[sys, highlightnode, fit=(dt1 process) (dt2 process),label={[below]north:{Energy Saving Warm Comfort DT}},xshift=.5em] (dt1-system) {};
\end{scope}

\begin{scope}[on background layer]
    \node[sys, fit=(temperature sensor)(room AT)(dt1-system)(heater),label={[below]north:{Energy Saving Warm Comfort Twin System}}] {};
\end{scope}


